Marginal Inference queries in Hidden Markov Models under context-free grammar constraints

The primary use of any probabilistic model involving a set of random variables is to run inference and sampling queries on it. Inference queries in classical probabilistic models is concerned by the computation of marginal or conditional probabilities of events given as an input. When the probabilistic model is sequential, more sophisticated marginal inference queries involving complex grammars may be of interest in fields such as computational linguistics and NLP. In this work, we address the question of computing the likelihood of context-free grammars (CFGs) in Hidden Markov Models (HMMs). We provide a dynamic algorithm for the exact computation of the likelihood for the class of unambiguous context-free grammars. We show that the problem is NP-Hard, even with the promise that the input CFG has a degree of ambiguity less than or equal to 2. We then propose a fully polynomial randomized approximation scheme (FPRAS) algorithm to approximate the likelihood for the case of polynomially-bounded ambiguous CFGs.

==> conclusion.tex <==
 

==> hardness.tex <==
\section{Hardness of computing likelihood of CFGs with constant ambiguity in HMMs}
Before presenting the algorithm for computing the likelihood of generating strings in an UCFGs from HMMs, we shall first examine the complexity of the same problem applied to the restricted class of CFGs with bounded constant ambiguity. \\
Define the counting problem:\\
\textbf{The k-CFG likelihood problem} \\
$\bullet$ \textbf{Instance:} A CFG G with constant ambiguity $k$, An HMM $A'$, a length $L > 0$ \\
$\bullet$ \textbf{Problem:} Compute $f_{A'}(L_{G} \cap \Sigma^{L})$ \\

When the ambiguity level $k$ is treated as a complexity parameter, the problem is computationaly intractable.
\begin{theorem}
 The k-CFG counting problem is \#P-Hard.
\end{theorem}
\begin{proof}
 The reduction is from the \#3SAT problem. The \#3SAT problem takes as input a propositional formula made of conjective form where each clause is made of 3 litterals and outputs the number of true assignments of the formula. \\
  Let $F = C_{1} \land C_{2} \land ..C_{k}$ be a propositional formula with $k$ clauses containing litterals from a set of $n$ boolean variables $\mathcal{X} = \{x_{i}\}_{i \in [n]}$, where each clause $C_{j}$ is a conjuction of 3 litterals written as $C_{j} = l_{1}^{(j)} \lor l_{2}^{(j)} \lor l_{3}^{(j)}$. Let \#F denote the number of true assignments of the formula. Without a loss of generality, we equip the set of variables $\mathcal{X}$ with a relation order associated with its index, which makes a one-to-one correspondance between the set of assignments and the set of strings $\{0,1\}^{n}$. A clause $C_{j}$ can be seen as a representation of a set of strings, denoted $L_{C_{j}}$, in $\{0,1\}^{n}$ corresponding to the set of assignments of the variables that satisfy the clause. For each clause $C_{j}$ in the formula, we construct a UCFG $G_{j}$ such that $L_{G_{j}} = \bar{L}_{C_{k}} \cap \Sigma^{n}$, i.e. $L_{G_{j}}$ represents the set of all strings corresponding to assignments that don't satisfy the clausse $C_{j}$. One can verify that the construction of a determinstic finite automaton of size $n$ representing the language $\bar{L}_{C_{k}} \cap \{0,1\}^{n}$ is straightforward. Converting a determinstic finite automaton of size $n$ to an equivalent determinstic context-free grammar (hence, unambiguous) of same size is also straightforward. Let $G$ be the CFG that represents the union of languages induced by $\{G_{j}\}_{j \in [k]}$. $G$ is constructed by introducing a new root symbol $S$, and adding new production rules such that for each grammar $G_{j}$, we have $S \rightarrow N.N'$ if $S_{j} \rightarrow N.N'$ where $S_{j}$ is the root symbol of $G_{j}$, and omitting the production rule $S_{j} \rightarrow NN'$ from the grammar $G$.   It's easy to check that this construction can be done in polynomial time with respect to $n$ and $k$. Moreover, $G$ satisfies two additional properties: (1) the ambiguity of the constructed CFG is less than $k$, (2) $w \not \in L_{G} \cap \{0,1\}^{n}$ if and only if the assignment of variables associated to $w$ satisfies the formula $F$. \\ 
  By (2), we have $\#F = |\bar{L}_{G}  \cap \Sigma^{n}| = 2^{n}. f_{A'}(\bar{L}_{G} \cap \{0,1\}^{n})$, where $A'$ is the trivial single-state HMM over the observation space $\{0,1\}$ such that $f_{A'}(w) = (\frac{1}{2})^{|w|}$. This is equivalent to $\#F = 2^{n}.(1 - f_{A'}(L_{G} \cap \{0,1\}^{n}))$. 
\end{proof}

==> introduction.tex <==
\section*{Introduction} 
 In practical applications, the primary use of any probabilistic model involving a set of random variables is to run inference and sampling queries on it: What would be the practical use of a probabilistic model in applications such as medical diagnosis and industrial maintenance without having an engin capable of computing conditional probabilities? An inference query\footnote{In this informal definition, we omit the case of decoding queries. Indeed, in the litterature of probabilistic modeling, the decoding problem is also referred to as an inference query. The decoding problem concerns the search of the most probable event among a collection of events.} can be defined informally as the computational problem of computing the probability of occurence of an event given as input. A sampling query is, on the other hand, the problem of generating a realization of the probabilistic model (potentially conditioning on the occurence of a given event). In classical bayesian modeling, it's well-known fact that exact inference in general bayesian networks is NP-Hard. Hence, most of the research effort in the field of bayesian was dedicated either to constrain the strutcture of bayesian networks to a more tractable, or to design approximate algorithms for making inference. \\
 Dynamical probabilistic modeling represents an important sub-field in the area of probabilistic models. Dynamical probabilistic models are dedicated to model sequential data.
 Due to their simplicity and ease of interpretation, hidden Markov models (HMMs) represent an important class of dynamic probabilistic models which enjoy an extensive research study. Due to their simplicity and ease of interpretation, HMMs were used in many applications such as bioinformatics, NLP, Speech and signal processing etc. With regard to making inference in HMMs, two widely popular algorithms were proposed in the litterature: The Forward-Backward and Viterbi algorithms. The former computes the probability of generating a given sequence, while the latter is dedicated to finding the most probable sequence (The decoding problem). Algorithms for more elaborate marginal queries can be obtained by observing that HMMs restricted to a bounded support are nothing but tree-structured bayesian networks. Luckily, exact inference in this class of probabilistic models is known to be tractable \cite{}. With this correspondance, one can readily obtain prrocedures to compute infix (or, more generally island) probabilities in HMMS by simple reduction. In most applications where HMMs are employed, this suite of marginal queries are proven to be sufficient for the task of interest. Yet, in fields such as computationnal linguistics, deeper structures of sequential data involving complex grammars are of interest. When HMMs are used in NLP tasks such as language modeling, we might be interested in extracting emergent grammars in the language model. Other concerns are related to the discriminative bias in language models. Indeed, recent studies showed that trained language models are subject of capturing negative stereotypes present in trained corpus \cite{}, a problem that raises a major ethical concern regarding the deployment of these models in real-case situations. Indeed,  more structurally complex patterns of sequential data are of interest. The goal of this article is to explore the perspective of widening the scope of marginal inference queries we can make on HMMs by putting into the picture languages generated by sophisticated grammars. Informally, the general problems can be stated as follows: \\
  let $\mathcal{R}$ be a class of machines/grammars inducing languages over the alphabet formed by the observation space of the HMM \footnote{A pattern language in our context refers to a set of sequences formed by the (discrete) observation space of the HMM}, given a HMM $M$, a machine/grammar $R \in \mathcal{R}$ and an integer $L>0$,
 \begin{itemize}
     \item \textbf{The $\mathcal{R}$-likelihood problem:} How to compute the likelihood of generating a sequence of length $L$ from $M$ that matches the pattern $R$?
     \item  \textbf{The $\mathcal{R}-$sampling problem:} How to sample strings of length $L$ from $M$ under the constraint that the generated string matches the pattern $R$?
 \end{itemize}
 $\mathcal{R}$ could represent a class of machines such as Nondeterministic or determinstic finite automata, or a class of grammars such as context-free grammars. Naturally, the complexity of these informatly stated problems will depend on the nature of $\mathcal{R}$.  \\ 
 These problems can be seen as a generalization of two classical problems in formal language theory: The counting and the uniform generation\cite{}\cite{}. For a class of machines/grammars $\mathcal{R}$, the counting problem asks about the number of words of a given length accepted by a machine/grammar $R \in \mathcal{R}$. The uniform generation aims at drawing uniformly at random strings of a given length in the support of accepted words of a machine/grammar in $\mathcal{R}$. These problems are easily reducible to problems of interest in this article, by choosing the HMM to be the trivial single-state model that assigns equal mass probability to all words at a given length. Therefore, by this straightforward reduction, one can show that the problem is $\#$P-Hard when $\mathcal{R}$ is the class of nondeterministic finite automata. A fortiori, same negative results hold for general context-free grammars. 
  Positive results of the $\mathcal{R}$-likelihood problem can be found in the litterature of computational linguistics interested in the closely rrelated problem of computing the weight of different classes of languages in stochastic grammars such as probabilistic context-free grammar and probabilistic finite automata (PFAs). Indeed, HMMs bounded to a given length can be efficiently converted to a PFA. Therefore, an algorithm designed for PFAs to compute the weight of languages represented by a class of machines/grammars $\mathcal{R}$ can be adapted to our problem. Earlier works adressed the problem of computing the weight of prefixes, suffixes and infixes in PFAs \cite{ana00}\cite{corazza81}. Recently, \cite{cognetta18, cognetta19} proposed an incremental algorithm for computing the weight of regular languages in PFAs, where the regular languages are represented by \textit{unambiguous} regular expressions. 
  it's well know that computing the prefix and suffix probabilities in probabilistic context-free grammars can be done in polynomial time\cite{lafferty91}\cite{stolcke95}. However, computing infix probabilities boils down to solving a non-linear system of equations whose exact solving is intractable \cite{corazza81}. The same issue was adressed in \cite{nederhof11}, where an efficient procedure of computing infix probability in probabilistic context-free grammars were proposed. Their method relies on intersecting the PCFG with an unambiguous finite automaton constructed from the infix string. Moreover, their method seems to be adapted easily to compute the weight of any regular language given in the form of an \textit{unambiguous} finite automaton in a PCFG. Later developments of this issue considered the more practically related question of computing infix probabilities in an online fashion. In two consecutive works \cite{cognetta18}\cite{cognetta19}, Cognetta et al. proposed an incremental algorithm for computing the weight of regular languages given in the form of a UFAs in a PFAs. Recently, Miller et al. \cite{miller21} proposed a procedure for sampling strings matching an \textit{unambiguous} regular expressions from uniform Matrix product state models, a particular class of probabilistic automata.   
 \\
The outline of this article is organized as follows. In setion 1, we present basic notations and definitions of different classes of machines/grammars that will be under study in the sequel. In section 2, 


==> introduction2.tex <==
Due to their simplicity and ease  of interpretation, Hidden Markov Models (HMMs) represent an important class of dynamic probabilistic models finding  its applications in many fields (bioinformatics, NLP, speech processing etc.). With regard to making inference in HMMs, two popular algorithms were proposed in the litterature: The forward algorithm and the Viterbi algorithm. The former computes the likelihood of generating a given sequence, while the latter is dedicated to the decoding problem. Algorithms for more elaborate marginal queries can be obtained by observing that HMMs restricted to a bounded support are nothing but tree-structured bayesian networks. Luckily, exact inference in this class of probabilistic models is known to be tractable (\cite{koller09}). With this correspondance, one can readily obtain procedures to compute infix (or, more generally island) probabilities in HMMs by straightforward reduction. In most applications where HMMs are employed, this suite of marginal inference queries proved to be sufficient for the task of interest. Yet, in fields such as computationnal linguistics, deeper structures of sequential data involving complex grammars are of interest. For instance, when HMMs are used in NLP tasks such as language modeling, we might be interested in extracting emergent grammars in the language model. Other concerns are related to the dicriminative bias in language models. Indeed, recent studies showed that trained language models are subject of capturing negative stereotypes present in the corpus used for training (\cite{sheng19}), a problem that raises a major ethical concern regarding the deployment of these models in real-case situations. The goal of this article is to explore the perspective of widening the scope of marginal inference queries we can make on HMMs by bringing to the picture languages generated by sophisticated grammars. Informally, let $\mathcal{R}$ be a class of machines/grammars inducing languages over the alphabet formed by the observation space of the HMM, the $\mathcal{R}$-likelihood problem can be stated as follows: Given an HMM $M$, a machine/grammar $R \in \mathcal{R}$ and an integer $L>0$: How to compute the likelihood of generating a sequence of length $L$ from $M$ accepted by $R$? \\
From the perspective of formal language theory, this problem can be seen as a generalization of the classical problem of counting the number of words accepted by a given machine/grammar. This counting problem is easily reducible to our problem, by choosing $M$ to be the trivial single-state HMM that assigns equal mass probability to all words at a given length. Therefore, by this straightforward reduction, one can show that the $\mathcal{R}$-likelihood problem is $\#$P-Hard when $\mathcal{R}$ is the class of nondeterministic finite automata (\cite{kannan95}). A fortiori, same negative results hold for general context-free grammars. \\
  Positive results of the $\mathcal{R}$-likelihood problem can be found in the litterature of computational linguistics interested in the closely related problem of computing the weight of different classes of languages in stochastic grammars such as probabilistic context-free grammars and probabilistic finite automata (PFAs). Indeed, HMMs bounded to a given length can be efficiently converted to a PFA. Therefore, an algorithm designed for PFAs to compute the weight of languages represented by a class of machines/grammars $\mathcal{R}$ can be adapted to our problem. Earlier works adressed the problem of computing the weight of prefixes, suffixes and infixes in PFAs (\cite{corazza81}, \cite{ana00}). Recently, \cite{cognetta18, cognetta19} proposed an incremental algorithm for computing the weight of regular languages in PFAs, where the regular languages are represented by \textit{unambiguous} regular expressions. \\
  In this article, we shall be interested in computing the likelihood of languages generated by different subclasses of  CFGs from HMMs (i.e. when $\mathcal{R}$ is a subclass of CFGs). The studied subsclasses will correspond to the hirerarchy of CFGs according to their ambiguity degree. The outline of the article is as follows: In Section 1, we present algebric descriptions of machines/grammars of interest in this article, that is CFGs and HMMs. In Section 2, we present a polynomial-time dynamic algorithm for solving the likelihood problem for the case of unambiguous context-free grammars (UCFG). In Section 3, we prove that the likelihood problem is NP-Hard even with the promise that the input CFG has an ambiguity degree less or equal to 2. We give afterwards a randomized procedure that provides FPRAS guarantees of the likelihood problem for the case of CFGs with polynomial ambiguity degree. 
